Transformers in Small Object Detection: A Benchmark and Survey of State-of-the-Art

Transformers have rapidly gained popularity in computer vision, especially in the field of object recognition and detection. Upon examining the outcomes of state-of-the-art object detection methods, we noticed that transformers consistently outperformed well-established CNN-based detectors in almost every video or image dataset. While transformer-based approaches remain at the forefront of small object detection (SOD) techniques, this paper aims to explore the performance benefits offered by such extensive networks and identify potential reasons for their SOD superiority. Small objects have been identified as one of the most challenging object types in detection frameworks due to their low visibility. We aim to investigate potential strategies that could enhance transformers' performance in SOD. This survey presents a taxonomy of over 60 research studies on developed transformers for the task of SOD, spanning the years 2020 to 2023. These studies encompass a variety of detection applications, including small object detection in generic images, aerial images, medical images, active millimeter images, underwater images, and videos. We also compile and present a list of 12 large-scale datasets suitable for SOD that were overlooked in previous studies and compare the performance of the reviewed studies using popular metrics such as mean Average Precision (mAP), Frames Per Second (FPS), number of parameters, and more. Researchers can keep track of newer studies on our web page, which is available at \url{https://github.com/arekavandi/Transformer-SOD}.

==> biblo.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.9in,clip,keepaspectratio]{Figures/Aref.eps}}]{Aref Miri Rekavandi}
	(Member, IEEE) received his B.Sc. degree in electrical engineering from KN Toosi University of Technology, Tehran, Iran, in 2013, M.Sc. degree in digital electronics engineering from Amirkabir University of Technology (Tehran Polytechnic), Tehran, Iran, in 2016, and Ph.D. degree in electrical and electronic engineering from The University of Melbourne, Melbourne, VIC, Australia, in 2021. He is a Research Fellow at the School of Physics, Maths and Computing, The University of Western Australia (2021-present) as well as a visiting researcher at Wellcome Centre for Integrative Neuroimaging, FMRIB Centre, University of Oxford, UK. His research interests include statistical signal and image processing, computer vision, medical imaging analysis, and pattern recognition.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.9in,clip,keepaspectratio]{Figures/Shima}}]{Shima Rashidi}
received her Ph.D. degree from the School of Computing and Information Systems, The University of Melbourne in 2022. Her Ph.D. was on modeling target detectability in natural scenes that mimics human behavior. She was a postdoctoral researcher in Intelligent Automation Systems at RMIT University, Melbourne (2021-2022).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.9in,clip,keepaspectratio]{Figures/Farid.jpg}}]{Farid Boussaid}
	received the M.S. and Ph.D. degrees in microelectronics from the National Institute of Applied Science (INSA), Toulouse, France, in 1996 and 1999, respectively. He joined Edith Cowan University, Perth, Australia, as a postdoctoral Research Fellow, and a Member of the Visual Information Processing research group in 2000. He joined the University of Western Australia, Crawley, Australia, in 2005, where he is currently a Professor. His current research interests include neuromorphic engineering, smart sensors, and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.9in,clip,keepaspectratio]{Figures/Saad.jpg}}]{Saad Jbabdi} is a Professor and
	head of Diffusion Analysis, Wellcome Centre for Integrative Neuroimaging (WIN) at University of Oxford, UK. His main research concerns Neuroscience, Diffusion MRI, Brain mapping, Tractography and Prefrontal cortex. His Neuroscience study frequently links to related topics such as Anatomy. His studies in Diffusion MRI integrate themes in fields like White matter, Amphetamine, Neuroimaging and Raclopride. His Brain mapping study integrates concerns from other disciplines, such as Positron emission tomography, Dopamine receptor, Dopamine, and Thalamus. His Tractography research focuses on Artificial intelligence and how it relates to Pattern recognition. His biological study spans a wide range of topics, including Voxel, Computer vision, Diffusion tensor tractography, and Randomized algorithms.
\end{IEEEbiography}

%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Karim}}]{Abd-Krim Seghouane}
%	 (Senior Member, IEEE) received the Ph.D. degree in signal processing and control from University Paris Sud (Paris XI), France, in 2003. From 2005 to 2012, he was a Researcher and subsequently a Senior Researcher with National ICT Australia (NICTA) Canberra Research Laboratory and an Adjunct Faculty with the College of Engineering and Computer Science, Australian National University (ANU). Prior to that, he was a Postdoctoral Researcher with INRIA Rocquencourt, France. He has been on the EEE Faculty with The University of Melbourne, since 2013. His research has been recognized via the Australian Research Council Future Fellowship. His research interests include statistical signal and image processing, including the application areas of medical imaging and physiological signal analysis. Dr. Seghouane is currently an Elected Member of the IEEE Signal Processing Society Machine Learning for Signal Processing Technical Committee (MLSPTC) elected first, in 2014 and re-elected, in 2017 for another term of three years. He was the Chair of the MLSP TC Data Competition Sub-committee, from 2014 to 2017. He was the General Co-Chair of the 2014 IEEE Workshop on Statistical Signal Processing, Gold Coast, Australia, the Data Competition Co-Chair of the 2017 and 2018 IEEE Workshop on Machine Learning for Signal Processing, Tokyo, Japan and Aalborg, Denmark, and the Organization Co-Chair of the 2017 IEEE International Symposium on Biomedical Imaging, Melbourne, Australia. He has served as an Associate Editor on the editorial board for the IEEE Transactions on Image Processing, from 2014 to 2018; and since 2018, serves as a Senior Editor of the area. He also serves on the editorial board of the IEEE Transactions on Signal Processing as an Associate Editor, since 2017.
%\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.6in,clip,keepaspectratio]{Figures/Wanli.jpg}}]{Wanli Ouyang} received the PhD degree in theDepartment of Electronic Engineering, The Chi-nese University of Hong Kong. He is now a pro-fessor at Shanghai AI lab, Shanghai, China, anda senior member of IEEE. His research interestsinclude image processing, computer vision, andpattern recognition.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.6in,clip,keepaspectratio]{Figures/Mohammed.jpg}}]{Mohammed Bennamoun} (Senior Member, IEEE) is Winthrop Professor in the Department of Computer Science and Software Engineering at UWA and is a researcher in computer vision, machine/deep learning, robotics, and signal/speech processing. He has published 4 books (available on Amazon, 1 edited book, 1 Encyclopedia article, 14 book chapters, 150+ journal papers, 250+ conference publications, 16 invited and keynote publications. His h-index is 69 and his number of citations is 22,100+ (Google Scholar). He was awarded 65+ competitive research grants, from the Australian Research Council, and numerous other Government, UWA and industry Research Grants. He successfully supervised 33+ PhD students to completion. He won the Best Supervisor of the Year Award at QUT (1998), and received award for research supervision at UWA (2008 and 2016) and Vice-Chancellor Award for mentorship (2016). He delivered conference tutorials at major conferences, including: IEEE Computer Vision and Pattern Recognition (CVPR 2016), Interspeech 2014, IEEE International Conference on Acoustics Speech and Signal Processing (ICASSP) and European Conference on Computer Vision (ECCV). He was also invited to give a Tutorial at an International Summer School on Deep Learning (DeepLearn 2017).
\end{IEEEbiography}
 
% \begin{thebibliography}{9}
% \bibitem{kisantal2019augmentation}
% M. Kisantal et al., `Augmentation for small object detection', \href{https://arxiv.org/abs/1902.07296v1}{ArXiv link}

% \bibitem{Oksuz}
% K. Oksuz, B. Cam, S. Kalkan and E. Akbas, "\href{https://www.computer.org/csdl/journal/tp/2021/10/09042296/1ikc4SuhD7q}{Imbalance Problems in Object Detection: A Review}" in IEEE Transactions on Pattern Analysis & Machine Intelligence, vol. 43, no. 10, pp. 3388-3415, 2021.

% \bibitem{Wu-review}
% X. Wu, D. Sahoo, S. C.H. Hoi,
% `\href{https://www.sciencedirect.com/science/article/pii/S0925231220301430?casa_token=nyAUsVXWl48AAAAA:6wG2zV-0koN56sn1Piq2wVN9_cF2piiGSY0k6At1eJCB3ywNgS3PDY1Ntvpx9j5wClcIgNArvdoS}{Recent advances in deep learning for object detection}',
% Neurocomputing,
% Volume 396,
% 2020,
% Pages 39-64.

% \bibitem{Liu-survey}
% Y. Liu et. al., `\href{http://www.joig.net/uploadfile/2021/1124/20211124052219501.pdf}{Survey of Video Based Small Target Detection}', Journal of Image and Graphics, Vol. 9, No. 4, December 2021

% \bibitem{zou-survey}
% Z. Zou et. al., `\href{https://arxiv.org/abs/1905.05055}{Object Detection in 20 Years: A Survey}', ArXiv.
% \end{thebibliography}
